Learning-Based Relaxation of Completeness Requirements for Data Entry Forms

Data entry forms use completeness requirements to specify the fields that are required or optional to fill for collecting necessary information from different types of users. However, some required fields may not be applicable for certain types of users anymore. Nevertheless, they may still be incorrectly marked as required in the form; we call such fields obsolete required fields. Since obsolete required fields usually have not-null validation checks before submitting the form, users have to enter meaningless values in such fields in order to complete the form submission. These meaningless values threaten the quality of the filled data. To avoid users filling meaningless values, existing techniques usually rely on manually written rules to identify the obsolete required fields and relax their completeness requirements. However, these techniques are ineffective and costly. In this paper, we propose LACQUER, a learning-based automated approach for relaxing the completeness requirements of data entry forms. LACQUER builds Bayesian Network models to automatically learn conditions under which users had to fill meaningless values. To improve its learning ability, LACQUER identifies the cases where a required field is only applicable for a small group of users, and uses SMOTE, an oversampling technique, to generate more instances on such fields for effectively mining dependencies on them. Our experimental results show that LACQUER can accurately relax the completeness requirements of required fields in data entry forms with precision values ranging between 0.76 and 0.90 on different datasets. LACQUER can prevent users from filling 20% to 64% of meaningless values, with negative predictive values between 0.72 and 0.91. Furthermore, LACQUER is efficient; it takes at most 839 ms to predict the completeness requirement of an instance.

==> pics/bayesian.tex <==

\tikzstyle{round_rect} = [rectangle, rounded corners, minimum width=1cm, minimum height=0.5 cm,text centered, draw=black, fill=white!30]
\tikzstyle{rect} = [rectangle, minimum width=1.5cm, minimum height=0.5cm, text centered, text width=1.5cm, draw=black, fill=white!30]
\tikzstyle{text_node} = [rectangle, minimum width=0.5cm, minimum height=0.35cm, text centered, text width=4cm, draw=white, fill= white!30]

\begin{minipage}[t]{\linewidth}
  \centering
  \scriptsize
  % \begin{tabular}[]{@{}m{18mm}@{\hspace{3pt}}b{15mm}@{\hspace{3pt}}b{20mm}@{\hspace{3pt}}b{20mm}}
  \begin{tabular}{ccc}
\begin{tikzpicture}[baseline,scale=0.7, every node/.style={scale=0.75},node distance=3mm, >=latex]

\node (A) [round_rect] {$\mathit{Company \ type}$};
\node (B) [round_rect, below= of A,xshift= 0.7cm] {$\mathit{Revenue}$};
\node (C) [round_rect, below= of A,xshift=-0.7cm] {$\mathit{Tax \ ID}$};


\draw [arrow,->] (A) -- (C);
\draw [arrow,->] (A) -- (B);
\draw [arrow,->] (B) -- (C);

\end{tikzpicture}
% \end{minipage}
% &
  
%   \begin{tabular}[t]{ c c}
%     \multicolumn{2}{c}{$P(A)$}\\
% 	\toprule
% 	$a$&$\Bar{a}$ \\
% 	\midrule
% 	0.2 & 0.8 \\
% 	\bottomrule
% 	\end{tabular}
    &%\hfill
      \multirow{3}{*}{%
	\begin{tabular}[b]{ c c c}
          \multicolumn{3}{c}{$P(\mathit{Revenue} \mid \mathit{Company \ type})$}\\
          \toprule
        \multirow{2.5}{*}{$\mathit{Company \ type}$} & \multicolumn{2}{c}{$\mathit{Revenue}$} \\ 
	\cmidrule{2-3}
	&$b$&$\Bar{b}$ \\
	\midrule
	$a$  & 0.4 & 0.6 \\
	$\Bar{a}$ & 0.1 & 0.9 \\
	\bottomrule
	\end{tabular}}
    &%\hfill
       \multirow{3}{*}{%
	\begin{tabular}[b]{c  c c  c}
          \multicolumn{4}{c}{$P(\mathit{Tax \ ID}\mid \mathit{Company \ type}, \mathit{Revenue})$} \\
          \toprule
	\multirow{2.5}{*}{$\mathit{Company \ type}$} & \multirow{2.5}{*}{$\mathit{Revenue}$} & \multicolumn{2}{c}{$\mathit{Tax \ ID}$} \\             
	\cmidrule{3-4}
	&&$c$&$\Bar{c}$\\
	\midrule
	$a $& $b $& 0.9 & 0.1  \\
	$a $& $\Bar{b}$ & 0.4 & 0.6 \\
	$\bar{a}$&$b$& 0.4 & 0.6 \\
	$\Bar{a}$ &$\Bar{b}$ & 0.1 & 0.9 \\
	\bottomrule
	\end{tabular}}\\ &&\\ 
   \begin{tabular}[b]{ c c}
    \multicolumn{2}{c}{$P(\mathit{Company \ type})$}\\
	\toprule
	$a$&$\Bar{a}$ \\
	\midrule
	0.2 & 0.8 \\
	\bottomrule
   \end{tabular}
&&\\    
\end{tabular}
\end{minipage}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/outline-introduction.tex <==
\begin{tabular}{p{1.25cm} p {0.5cm}p{5.25cm }p{5.25cm}}
	\toprule
	&&\multicolumn{1}{c} {LAFF paper~\cite{belgacem2022machine}} &\multicolumn{1}{c} {this paper}\\
	\midrule
	
	

	
\multicolumn{2}{ l}{\multirow{25}{*}{Introduction} } & 
\vspace{-0.5\baselineskip}
\begin{itemize}
	\item Data entry and form filling
	\item The burden of form filling on users (form filling and data entry forms)
	 \item The importance of data entry error prevention and existing works
	 \item Data entry errors in categorical fields  (main causes)
	 \item Existing form-filling approaches and their limitations
	 \item Overview of our solution LAFF
	 \item Main phases of LAFF
	 \item Summary of the main results of LAFF
	 \item Contributions
	 
\end{itemize}
\nointerlineskip
&
\vspace{-0.5\baselineskip}
\begin{itemize}
	\item Data entry forms and completeness requirements
	\item Data entry requirement changes and obsolete required fields
	\item Meaningless values phenomenon 
	\item The effect of meaningless values
	\item Existing works on adaptive forms
	\item Overview of  our solution \approach
	\item Main phases of \approach
	\item Similarities between \approach and LAFF
	\item Summary of the main results of \approach
	\item Contributions
\end{itemize}
\nointerlineskip \\
\cmidrule{1-4}



\end{tabular}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/outline-sec2.tex <==
\begin{tabular}{p{1.25cm} p {0.5cm}p{5.25cm }p{5.25cm}}
	\toprule
	\multicolumn{1}{c} {subsection title} &&\multicolumn{1}{c}{LAFF paper~\cite{belgacem2022machine}} &\multicolumn{1}{c}{this paper}\\
	\midrule
	
	

	
\multicolumn{2}{ l}{\multirow{10}{*}{Data entry forms} } & 
\vspace{-0.5\baselineskip}
\begin{itemize}
	\item Data entry forms and types of fields (textual, categorical, etc.)
	 
\end{itemize}
\nointerlineskip
&
\vspace{-0.5\baselineskip}
\begin{itemize}
	\item Data entry form fields and their completeness requirements (optional, required)
	\item Conditional required fields 
	\item Framing the targeted data entry forms
\end{itemize}
\nointerlineskip \\
\cmidrule{1-4}

\multicolumn{2}{ l}{\multirow{12}{*}{Motivating example} } & 
\vspace{-0.5\baselineskip}
\begin{itemize}
	\item Two motivating examples from the biomedical and the banking domains illustrating the main challenges of form filling 
	\item Problems of existing solutions (e.g., web browser plug-ins for form filling)
	
\end{itemize}
\nointerlineskip
&
\vspace{-0.5\baselineskip}
\begin{itemize}
	\item One motivating example (data entry form of an energy provider company)
	\item Effect of meaningless values
	\item Example of simple but not practical solutions to address the meaningless values (rule-based solutions and dictionary-based solutions)
\end{itemize}
\nointerlineskip \\
\cmidrule{1-4}



\multicolumn{2}{ l}{\multirow{8}{*}{Challenges} } & 
\vspace{-0.5\baselineskip}
\begin{itemize}
	\item Definition of the form-filling problem
	\item Application to the running example (opening of a bank account)
	
\end{itemize}
\nointerlineskip
&
\vspace{-0.5\baselineskip}
\begin{itemize}
	\item Definition of the completeness requirement relaxation problem
	\item Framing the problem definition scope
	\item Application to running example (opening an
	account for business customers in the energy provider information system)

	
\end{itemize}
\nointerlineskip \\
\cmidrule{1-4}


\multicolumn{2}{ l}{\multirow{8}{*}{Problem definition} } & 
\vspace{-0.5\baselineskip}
\begin{itemize}
	\item Main idea of form-filling approaches
	\item Arbitrary filling order
	\item Partially filled forms
	
\end{itemize}
\nointerlineskip
&
\vspace{-0.5\baselineskip}
\begin{itemize}
	\item The need for a complete set of rules for existing relaxing completeness requirements approaches
	\item The evolving nature of data entry forms
	
	
\end{itemize}
\nointerlineskip \\
\cmidrule{1-4}




\end{tabular}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/preprocessing.tex <==


\newcommand{\tikzmark}[2]{
	\tikz[overlay,remember picture,baseline] 
	\node [anchor=base] (#1) {$#2$};%
}

\newcommand{\DrawVLine}[3][]{%
	\begin{tikzpicture}[overlay,remember picture]
		\draw[shorten <=0.3ex, #1] (#2.north) -- (#3.south);
	\end{tikzpicture}
}

\newcommand{\DrawCircle}[1][]{%
	\begin{tikzpicture}[overlay,remember picture]
		\draw[black,fill=black] (0,0.5ex) circle (0.5ex);
	\end{tikzpicture}
}

\newcommand{\DrawRec}[1][]{%
	\begin{tikzpicture}[overlay,remember picture]
		\draw[black,fill=black] (-0.5ex,0) rectangle ++(1ex, 1ex);
	\end{tikzpicture}
}

\newcommand{\DrawTriangle}[1][]{%
	\begin{tikzpicture}[overlay,remember picture]
		\filldraw[fill=black] (90:1.2ex) -- (170:0.7ex) -- (10:0.7ex) --cycle;
	\end{tikzpicture}
}

\tikzstyle{round_rect} = [rectangle, rounded corners, minimum width=1.5cm, minimum height=0.5 cm,text centered, draw=black, fill=white!30]

\tikzstyle{rect} = [rectangle, minimum width=1.5cm, minimum height=0.8cm, text centered, text width=1.5cm, draw=black, fill=white!30]

\tikzstyle{text_node} = [rectangle, minimum width=0.5cm, minimum height=0.35cm, text centered, text width=4cm, draw=white, fill= white!30]
\resizebox{0.68\textwidth}{!}{
\begin{tikzpicture}
	
	\node (tab1) [shape=rectangle,draw=white] {
		\scriptsize
		\begin{tabular}{ccccc}
			\toprule
			
		\textbf{$f_1$: Company}&\textbf{$f_2$: Monthly}&\multirow{2}{*}{\textbf{$f_3$: Company type}}&\textbf{$f_4$: Field of }&\multirow{2}{*}{\textbf{$f_5$: Tax ID}}\\
		\textbf{name}&\textbf{ revenue}&&\textbf{ activity}&\\
		\emph{(Textual)}&\emph{(Numerical)}&\emph{(Categorical)}&\emph{(Categorical)}&\emph{(Textual)}\\
			\midrule
			
			{\color{gray}\text{UCI}$\rightarrow$} Required &{\color{gray}20$\rightarrow$}[20,22) &Large enterprise  &Real estate&T190 \\
			\midrule
			{\color{gray}{KDL $\rightarrow$}} Required&{\color{gray}21$ \rightarrow$}[20,22) &Large enterprise   &Manufacturing&T201  \\ 
			\midrule
			{\color{gray}{EoP}$\rightarrow$} Required&{\color{gray}@$\rightarrow$}Optional&Large enterprise &  Manufacturing& T200   \\ 
			\midrule
			{\color{gray}{UNI}$\rightarrow$} Required &{\color{gray}39$\rightarrow$}[39,41)&NPO&Education &{\color{gray}n/a$\rightarrow$}Optional \\ 

			
			\bottomrule
		\end{tabular}
		%	\DrawVLine[black, thick]{topC1}{bottomC1}
	};
\end{tikzpicture}}


==> pics/smote.tex <==

%\tikzstyle{round_rect} = [rectangle, rounded corners, minimum width=1cm, minimum height=0.5 cm,text centered, draw=black, fill=white!30]
%\tikzstyle{rect} = [rectangle, minimum width=1.5cm, minimum height=0.5cm, text centered, text width=1.5cm, draw=black, fill=white!30]
%\tikzstyle{text_node} = [rectangle, minimum width=0.5cm, minimum height=0.35cm, text centered, text width=4cm, draw=white, fill= white!30]

\newcommand{\tikzmark}[2]{
	\tikz[overlay,remember picture,baseline] 
	\node [anchor=base] (#1) {$#2$};%
}

\newcommand{\DrawVLine}[3][]{%
	\begin{tikzpicture}[overlay,remember picture]
		\draw[shorten <=0.3ex, #1] (#2.north) -- (#3.south);
	\end{tikzpicture}
}

\newcommand{\DrawCircle}[1][]{%
	\begin{tikzpicture}[overlay,remember picture]
		\draw[black,fill=black] (0,0.5ex) circle (0.5ex);
	\end{tikzpicture}
}

\newcommand{\DrawRec}[1][]{%
	\begin{tikzpicture}[overlay,remember picture]
		\draw[black,fill=black] (-0.5ex,0) rectangle ++(1ex, 1ex);
	\end{tikzpicture}
}

\newcommand{\DrawTriangle}[1][]{%
	\begin{tikzpicture}[overlay,remember picture]
		\filldraw[fill=black] (90:1.2ex) -- (170:0.7ex) -- (10:0.7ex) --cycle;
	\end{tikzpicture}
}

\tikzstyle{round_rect} = [rectangle, rounded corners, minimum width=1.5cm, minimum height=0.5 cm,text centered, draw=black, fill=white!30]

\tikzstyle{rect} = [rectangle, minimum width=1.5cm, minimum height=0.8cm, text centered, text width=1.5cm, draw=black, fill=white!30]

\tikzstyle{text_node} = [rectangle, minimum width=0.5cm, minimum height=0.35cm, text centered, text width=4cm, draw=white, fill= white!30]
\resizebox{0.68\textwidth}{!}{
	\begin{tikzpicture}
		
		\node (tab1) [shape=rectangle,draw=white] {
			\scriptsize
%			\begin{tabular}{cccc}
%				\toprule
%				
%				\textbf{}&\textbf{$f_2$: Monthly}&\textbf{$f_4$: Field of }&\multirow{2}{*}{\textbf{$f_3$: Target}}\\
%				\textbf{}&\textbf{ revenue}&\textbf{activity}&{}\\
%		
%				\midrule
%				
%			   i1&39&NPO&Optional\\
%				i2&42&NPO&Optional\\
%				i3&25&NPO&Optional\\
%				i4&100&LE&Required\\
%				i5&150&LE&Required\\
%				i6&200&LE&Required\\
%				i7&400&LE&Required\\
			\begin{tabular}{ccc}
			\toprule
			
			\textbf{}&\textbf{$f_2$: Monthly}&\multirow{2}{*}{\textbf{$f_3$: Target}}\\
			\textbf{}&\textbf{revenue}&{}\\
			
			\midrule
			
			i1&39&Optional\\
			i2&42&Optional\\
			i3&25&Optional\\
			i4&100&Required\\
			i5&150&Required\\
			i6&200&Required\\
			i7&400&Required\\
				\bottomrule
			\end{tabular}
			%	\DrawVLine[black, thick]{topC1}{bottomC1}
		};
	
	
	\node (tab2) [shape=rectangle,draw=white, right =of  tab1] {
		\scriptsize
%		\begin{tabular}{cccc}
%			\toprule
%			
%			\textbf{}&\textbf{$f_2$: Monthly}&\textbf{$f_4$: Field of }&\multirow{2}{*}{\textbf{$f_3$: Target}}\\
%			\textbf{}&\textbf{ revenue}&\textbf{activity}&{}\\
%			
%			\midrule
%			
%			i1&39&NPO&Optional\\
%			i2&42&NPO&Optional\\
%			i3&25&NPO&Optional\\
%			i4&100&LE&Required\\
%			i5&150&LE&Required\\
%			i6&200&LE&Required\\
%			i7&400&LE&Required\\
%			i8&40&NPO&Optional\\

\begin{tabular}{ccc}
	\toprule
	
	\textbf{}&\textbf{$f_2$: Monthly}&\multirow{2}{*}{\textbf{$f_3$: Target}}\\
	\textbf{}&\textbf{revenue}&{}\\
	
	\midrule
	
	i1&39&Optional\\
	i2&42&Optional\\
	i3&25&Optional\\
	i4&100&Required\\
	i5&150&Required\\
	i6&200&Required\\
	i7&400&Required\\
    i8&40&Optional\\

			\bottomrule
		\end{tabular}
		%	\DrawVLine[black, thick]{topC1}{bottomC1}
		
	
	};
\draw[arrow,->] (tab1)--node[anchor=south] {\scriptsize SMOTE}(tab2);
\end{tikzpicture}}


==> pics/table-diff.tex <==
\begin{tabular}{p{1.25cm} p {0.5cm}p{5.25cm }p{5.25cm}}
	\toprule
	&&\multicolumn{1}{c} {LAFF} &\multicolumn{1}{c} {\approach}\\
	\midrule
	
	
	\multicolumn{2}{ l}{\multirow{2.5}{*}{Goal} } & 
	 \vspace{-0.5\baselineskip}
	\begin{itemize}
	\item Providing form-filling suggestions for the values to be filled in categorical fields
	\end{itemize}
	\nointerlineskip
	&
	\vspace{-0.5\baselineskip}
	\begin{itemize}
		\item Determining the completeness requirements of form
	\end{itemize}
    \nointerlineskip \\
	\cmidrule{1-4}
	
	\multicolumn{2}{ l}{\multirow{3}{*}{Challenge}} & 
	 \vspace{-0.5\baselineskip}
	\begin{itemize}
	  \item Arbitrary filling order
	\item Partial filling
	\end{itemize}
	\nointerlineskip
	& 
	\vspace{-0.5\baselineskip}
	\begin{itemize}
		\item Arbitrary filling order
		\item Partial filling 
		\item Highly imbalanced dataset
	\end{itemize}
	\nointerlineskip \\
	\cmidrule{1-4}
	
	\multicolumn{2}{ l}{\multirow{3}{*}{Preprocessing}} &  
	\vspace{-0.5\baselineskip}
	\begin{itemize}
	 \item  Textual fields are removed
	\end{itemize}
	\nointerlineskip 
	&
	\vspace{-0.5\baselineskip}
	\begin{itemize}
	\item Values in textual fields are transformed into binary values (``Required'' or ``Optional'')
	\item Meaningless values are identified and replaced with the value ``Optional''
	
	\end{itemize}
\nointerlineskip  \\
	\cmidrule{1-4}
	
	\multicolumn{2}{ l}{\multirow{4}{*}{Model building}} &  
	\vspace{-0.5\baselineskip}
	\begin{itemize}
	  \item Creates $k+1$ models including a global model and $k$ local models (one model for each cluster of data)
	  %\item A global model, built on the whole training data 
	 
	 	\end{itemize}
 \nointerlineskip  
	& 
	\vspace{-0.5\baselineskip}
	\begin{itemize}
	\item  Creates $n$ models, one model for each field (target)
	%\item Apply SMOTE on the training data
  \end{itemize}
  \nointerlineskip   \\
	\cmidrule{1-4}
	\multirow{8}{*}{Prediction} & \multirow{3}{*}{Target} &
	\vspace{-0.5\baselineskip}
	\begin{itemize}
		 \item Categorical field
		 \item LAFF can predict the value for both optional and required fields
	\end{itemize}
	 \nointerlineskip  
	  & 
	  \vspace{-0.5\baselineskip}
	  \begin{itemize}
         \item All textual, numerical, and categorical fields can be targets
		 \item Required field
		\end{itemize}
	 \nointerlineskip  
	  \\ \cline{2-4}
	
	& \multirow{4}{*}{Endorser} &
	 \vspace{-0.5\baselineskip}
	\begin{itemize}
	     \item Use two heuristics based on prediction confidence and dependencies between filled fields and the target
		 \item The value of the threshold is manually decided based on domain expertise
		 	\end{itemize}
	 \nointerlineskip & 
	 \vspace{-0.5\baselineskip}
	 \begin{itemize}
		\item The endorser is based only on the prediction confidence
		\item The value of the threshold is automatically determined during the threshold determination
	\end{itemize}
\nointerlineskip \\ 
		
	
	%	\emph{Challenges} &The fraction of correctly detected anomalies among all the anomalous instances~\cite{rashidi2011anomaly}.
	%&7\\
	%	\cmidrule{1-3}
	%	 \emph{Preprocessing} &The fraction of correctly predicted anomalies among the total number of predictions.~\cite{rashidi2011anomaly} &3\\ 
	%	 \cmidrule{1-3}
	%	\emph{Model building} &The number of correctly detected anomalies.
	%	&2\\ 
	%	 \cmidrule{1-3}
	%
	%	\emph{Prediction} &The harmonic mean of precision and recall~\cite{avazpour2014dimensions}.
	%	&1\\
	%	%\cmidrule{1-3}
	%	
	
	\bottomrule
\end{tabular}


%\begin{tabular}{p{1.25cm} p {0.5cm}p{5.25cm }p{5.25cm}}
%	\toprule
%	&&\begin{center}
%		LAFF
%	\end{center}&\begin{center}\approach \end{center}\\
%	\midrule
%    
%  
%	\multicolumn{2}{ l}{Goal } & \begin{itemize}
%		\item Suggest values to be filled in data entry from
%	\end{itemize}
%	 &  \begin{itemize}
%	 	\item Relax completeness requirements of data entry form
%	 \end{itemize} \\
%	\cmidrule{1-4}
%	
%	\multicolumn{2}{ l}{Challenge} & \begin{itemize}
%		\item The arbitrary order of filling
%		\item Partial filling
%	\end{itemize}
%	& \begin{itemize}
%		\item The arbitrary order of filling
%		\item Partial filling
%		\item Imbalanced data 
%	\end{itemize}\\
%	\cmidrule{1-4}
%	
%	\multicolumn{2}{ l}{Preprocessing} &  \begin{itemize}
%		\item Textual fields are removed
%	\end{itemize}
%	& \begin{itemize}
%		\item Identify meaningless values
%		\item All values in textual fields are transformed into ``required'' or ``optional''
%	\end{itemize}\\
%	\cmidrule{1-4}
%	
%	\multicolumn{2}{ l}{Model building} &  \begin{itemize}
%		\item A global model, built on the whole training data
%		\item Several local models, built on subsets of training data with similar characteristics
%	\end{itemize}
%	& \begin{itemize}
%		\item Apply SMOTE on the training data
%		\item One model for each target
%	\end{itemize} \\
%	\cmidrule{1-4}
%	
%	
%	\multirow{10}{*}{Prediction} & \multirow{5}{*}{Target} &
%	\begin{itemize}
%		\item Need to be a categorical field
%		\item LAFF can predict the value for both optional and required fields
%	\end{itemize}  & 
%	\begin{itemize}
%		\item All textual, numerical, and categorical fields can be targets
%		\item Need to be a required field
%	\end{itemize}  \\ \cline{2-4}
%	
%	& \multirow{5}{*}{Endorser} &\begin{itemize}
%		\item Use two heuristics based on prediction confidence and dependencies between fields
%		\item The value of threshold is decided by the designer
%	\end{itemize}   & 
%
%	\begin{itemize}
%		\item The endorser is based on the prediction confidence only
%		\item The value of the threshold is automatically determined
%	\end{itemize} \\ 
%	
%	
%%	\emph{Challenges} &The fraction of correctly detected anomalies among all the anomalous instances~\cite{rashidi2011anomaly}.
%%&7\\
%%	\cmidrule{1-3}
%%	 \emph{Preprocessing} &The fraction of correctly predicted anomalies among the total number of predictions.~\cite{rashidi2011anomaly} &3\\ 
%%	 \cmidrule{1-3}
%%	\emph{Model building} &The number of correctly detected anomalies.
%%	&2\\ 
%%	 \cmidrule{1-3}
%%
%%	\emph{Prediction} &The harmonic mean of precision and recall~\cite{avazpour2014dimensions}.
%%	&1\\
%%	%\cmidrule{1-3}
%%	
%	
%\bottomrule
   %  \end{tabular}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/table-rq-applicability.tex <==
\pgfplotstabletypeset[
every head row/.style={
	before row={%
		\toprule
		\multirow{2.5}{*}{}&\multirow{2.5}{*}{Alg.}&\multicolumn{4}{c}{Sequential}&\multicolumn{4}{c}{Partial Random}&\multirow{1}{*}{Train}&\multicolumn{2}{c}{Predict (\si{\milli\s})}\\
		\cmidrule(r){3-6}
		\cmidrule(l){7-10}
	},
	after row=\midrule,
},
every last row/.style={
	after row=\bottomrule
},
every nth row={3}{before row=\midrule},
columns/Dataset/.style ={column name=}, 
columns/Algorithm/.style ={column name=}, 
columns/Prec-S1/.style={column name=Prec}, 
columns/Rec-S1/.style ={column name=Rec},
columns/NPV-S1/.style ={column name=NPV},
columns/Spec-S1/.style ={column name=Spec},
columns/Prec-R1/.style={column name=Prec}, 
columns/Rec-R1/.style ={column name=Rec},
columns/NPV-R1/.style ={column name=NPV},
columns/Spec-R1/.style ={column name=Spec},
columns/Train/.style ={column name=(\si{\s})},
columns/P-Avg/.style ={column name=avg},
columns/P-Range/.style ={column name=min--max},
col sep=comma,
string type,
]{data/rq-applicability.csv}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/table-rq-component.tex <==
\resizebox{\columnwidth}{!}{%
	\pgfplotstabletypeset[
	every head row/.style={
		before row={%
			\toprule
			\multirow{4.5}{*}{ID}&\multicolumn{2}{c}{\multirow {2.5}{*}{Module}}&\multicolumn{8}{c}{NCBI}&\multicolumn{8}{c}{PEIS}\\
			\cmidrule(lr){4-11}
			\cmidrule(lr){12-19}
			&&&\multicolumn{4}{c}{Sequential}&\multicolumn{4}{c}{Partial
                          Random}&\multicolumn{4}{c}{Sequential}&\multicolumn{4}{c}{Partial
                          Random}\\
			\cmidrule(lr){2-3}
			\cmidrule(lr){4-7}
			\cmidrule(lr){8-11}
			\cmidrule(lr){12-15}
			\cmidrule(l){16-19}
		},
		after row=\midrule,
	},
	every last row/.style={
		after row=\bottomrule
	},
	columns/ID/.style = {column name=},
	columns/Local/.style = {column name=S},
	columns/Filter/.style = {column name=E},
	columns/PRE-S1/.style ={column name=Prec}, 
	columns/REC-S1/.style={column name=Recall},  
	columns/NPV-S1/.style={column name=NPV},  
	columns/SPE-S1/.style={column name=Spec},  
	columns/PRE-R1/.style ={column name=Prec}, 
	columns/REC-R1/.style={column name=Recall},  
	columns/NPV-R1/.style={column name=NPV},  
	columns/SPE-R1/.style={column name=Spec},   
	columns/PRE-S2/.style ={column name=Prec}, 
	columns/REC-S2/.style={column name=Recall},  
	columns/NPV-S2/.style={column name=NPV},  
	columns/SPE-S2/.style={column name=Spec},  
	columns/PRE-R2/.style ={column name=Prec}, 
	columns/REC-R2/.style={column name=Recall},  
	columns/NPV-R2/.style={column name=NPV},  
	columns/SPE-R2 /.style={column name=Spec},  
	col sep=comma,
	string type,
	]{data/rq-component.csv}
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

